ASPEST: Bridging the Gap Between Active Learning and Selective Prediction

Selective prediction aims to learn a reliable model that abstains from making predictions when uncertain. These predictions can then be deferred to humans for further evaluation. As an everlasting challenge for machine learning, in many real-world scenarios, the distribution of test data is different from the training data. This results in more inaccurate predictions, and often increased dependence on humans, which can be difficult and expensive. Active learning aims to lower the overall labeling effort, and hence human dependence, by querying the most informative examples. Selective prediction and active learning have been approached from different angles, with the connection between them missing. In this work, we introduce a new learning paradigm, active selective prediction, which aims to query more informative samples from the shifted target domain while increasing accuracy and coverage. For this new paradigm, we propose a simple yet effective approach, ASPEST, that utilizes ensembles of model snapshots with self-training with their aggregated outputs as pseudo labels. Extensive experiments on numerous image, text and structured datasets, which suffer from domain shifts, demonstrate that ASPEST can significantly outperform prior work on selective prediction and active learning (e.g. on the MNIST$\to$SVHN benchmark with the labeling budget of 100, ASPEST improves the AUACC metric from 79.36% to 88.84%) and achieves more optimal utilization of humans in the loop.

==> discussion.tex <==

\section{Discussion}
\label{sec:discussion}

Since our work is the first to study active selective prediction, we begin with the simple but efficient supervised training setting (i.e., use supervised training objectives when fine-tuning the model on the selected labeled test data). Note that the supervised training objectives can be easily extended to the semi-supervised training objectives that utilize unsupervised domain adaption (UDA) techniques. To demonstrate this, we evaluate DE with UDA and ASPEST with UDA in Appendix~\ref{app:train-uda} to show the effect of incorporating UDA techniques into training. Although UDA methods could improve the target test accuracy, their performance may not be stable across different kinds of distribution shifts and sometimes they can even yield accuracy degradation~\citep{johansson2019support,sagawa2021extending}. In our experiments, we also observe that the state-of-the-art UDA methods DANN~\citep{ganin2016domain} and CDAN~\citep{long2018conditional} are not stable in improving selective prediction performance across different datasets and different labeling budgets. One limitation of our work is that we don't fully explore the potentials of UDA. However, better UDA techniques can be easily incorporated into ASPEST to enhance its overall performance.
